Learning to sample in Cartesian MRI

Despite its exceptional soft tissue contrast, Magnetic Resonance Imaging (MRI) faces the challenge of long scanning times compared to other modalities like X-ray radiography. Shortening scanning times is crucial in clinical settings, as it increases patient comfort, decreases examination costs and improves throughput. Recent advances in compressed sensing (CS) and deep learning allow accelerated MRI acquisition by reconstructing high-quality images from undersampled data. While reconstruction algorithms have received most of the focus, designing acquisition trajectories to optimize reconstruction quality remains an open question. This thesis explores two approaches to address this gap in the context of Cartesian MRI. First, we propose two algorithms, lazy LBCS and stochastic LBCS, that significantly improve upon G\"ozc\"u et al.'s greedy learning-based CS (LBCS) approach. These algorithms scale to large, clinically relevant scenarios like multi-coil 3D MR and dynamic MRI, previously inaccessible to LBCS. Additionally, we demonstrate that generative adversarial networks (GANs) can serve as a natural criterion for adaptive sampling by leveraging variance in the measurement domain to guide acquisition. Second, we delve into the underlying structures or assumptions that enable mask design algorithms to perform well in practice. Our experiments reveal that state-of-the-art deep reinforcement learning (RL) approaches, while capable of adaptation and long-horizon planning, offer only marginal improvements over stochastic LBCS, which is neither adaptive nor does long-term planning. Altogether, our findings suggest that stochastic LBCS and similar methods represent promising alternatives to deep RL. They shine in particular by their scalability and computational efficiency and could be key in the deployment of optimized acquisition trajectories in Cartesian MRI.

==> figures/gan/tables/bakker_knee_table.tex <==
\begin{figure}[h]
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
         \toprule
        \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
        \midrule
        \textbf{Random} & $24.22$ & $20.68$ \\
        \textbf{LtH} & $24.25$ & $23.63$\\
        \textbf{LBCS} & $24.57$& $23.82$\\
        \textbf{NA Oracle}& $24.56$& $23.82$\\           
        \textbf{Bakker} & $24.37$& $22.50$ \\
        \bottomrule
        \end{tabular}
        \captionof{table}{Average PSNR test set AUC (one AUC per image) on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_psnr}     \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
            \toprule
           \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
           \midrule
            \textbf{Random}& $0.6251$& $0.5557$ \\
            \textbf{LtH}& $0.6073$& $0.5687$\\
            \textbf{LBCS}& $0.6355$& $0.5894$\\
            \textbf{NA Oracle}& $0.6355$& $0.5886$\\           
            \textbf{Bakker}& $0.6387$& $0.6153$ \\
           \bottomrule
           \end{tabular}
           \captionof{table}{Average SSIM test set AUC (one AUC per image) on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_ssim} 
    \end{center}
    \end{minipage}
    \end{figure}
    
    
    
    \begin{figure}[h]
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
         \toprule
        \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
        \midrule
        \textbf{Random} & $24.84$ & $21.66$ \\
        \textbf{LtH} & $24.81$ & $24.81$\\
        \textbf{LBCS} & $25.40$& $25.40$\\
        \textbf{NA Oracle}& $25.39$& $25.40$\\           
        \textbf{Bakker} & $25.18$& $24.60$ \\
        \bottomrule
        \end{tabular}
        \captionof{table}{Average PSNR at $25\%$ on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_psnr_25}     \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
            \toprule
           \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
           \midrule
            \textbf{Random}& $0.6896$& $0.6589$ \\
            \textbf{LtH}& $0.6586$& $0.6586$\\
            \textbf{LBCS}& $0.7086$& $0.7095$\\
            \textbf{NA Oracle}& $0.7099$& $0.7097$\\           
            \textbf{Bakker}& $0.7165$& $0.7400$ \\
           \bottomrule
           \end{tabular}
           \captionof{table}{Average SSIM at $25\%$ on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_ssim_25} 
    \end{center}
    \end{minipage}
    \end{figure}

==> figures/gan/tables/cifar_baseline.tex <==
\begin{center}
\begin{minipage}[t]{0.7\textwidth}

\input{files/gan/tables/cifar_image}
\end{minipage}\hfill
\end{center}

==> figures/gan/tables/cifar_image.tex <==
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lll|ccc}
    \toprule
    Algorithm & Model & Architecture & PSNR [dB]$~(\uparrow)$  &SSIM $(\uparrow)$& Accuracy  $ [\%]~(\uparrow)$\\
    \midrule
    \multirow{2}{*}{VDS} 
    & NC & ResUNet& $9.32\pm 0.70$  & $0.11\pm0.03$ & $0.10\pm 0.17$ \\
    & WGAN & ResUNet & $8.72\pm 0.62$  & $0.09\pm 0.03$ & $0.10\pm 0.17$ \\    
    \midrule
    \multirow{2}{*}{VDS}  & Recon. & ResUNet& $6.73\pm 0.51$  & $0.09\pm 0.02$ & $0.11\pm0.17$  \\
     & Recon. & c-ResNet& $ 11.79 \pm 0.72$  & $0.13 \pm 0.03$& $0.10\pm0.16$ \\
    \midrule
    \multirow{2}{*}{\begin{minipage}{1cm}GAS (Ours)\end{minipage}}
     & NC & ResUNet& $14.36 \pm 1.89$  & $0.55\pm 0.08$ & $\mathbf{0.27 \pm 0.22}$ \\
     & WGAN & ResUNet& $\mathbf{15.26\pm 2.34}$  & $\mathbf{0.57 \pm 0.09}$ & $0.21 \pm 0.18$ \\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC (one AUC per image) with standard deviation on CIFAR10, in image domain. This was computed on a subset of the test set.}\label{tab:comp_cifar_i}    

==> figures/gan/tables/knee_extended_table.tex <==
\begin{figure}[h]
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
         \toprule
        \multirow{1}{*}{\textbf{Policy}}& \multicolumn{2}{c}{\textbf{Model}}\\
        \cmidrule{2-3} & AO & Zhang\\
        \midrule
        \textbf{LtH} & $32.38$ & $31.97$\\
        \textbf{VDS} & $32.17$ & $31.29$ \\
        \textbf{LtH-VDS} & $32.94$ & $31.94$ \\
        \textbf{LBCS} & $33.40$& $32.13$\\
        \textbf{Zhang Evaluator} & $31.14$& $31.58$\\
        \textbf{Bakker} & $32.39$& $31.49$ \\
        \textbf{Uncertainty (Ours)} & $32.36$& $31.75$\\
        \midrule
        \textbf{0-step MSE Oracle} & $32.58$ & $32.18$\\
        \textbf{1-step SSIM Oracle} & $32.23$ & $32.24$\\
        \bottomrule
        \end{tabular}
        \captionof{table}{Average PSNR test set AUC (one AUC per image) on Knee 128.}\label{tab:comp_knee_psnr} 
    \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
            \toprule
           \multirow{1}{*}{\textbf{Policy}}& \multicolumn{2}{c}{\textbf{Model}}\\
           \cmidrule{2-3} & AO & Zhang\\
           \midrule
           \textbf{LtH}& $0.785$& $0.813$\\
           \textbf{VDS}& $0.792$& $0.795$ \\
           \textbf{LtH-VDS}& $0.805$ & $0.808$ \\
           \textbf{LBCS}& $0.815$& $0.813$\\
           \textbf{Zhang Evaluator}& $0.759$& $0.802$\\
           \textbf{Bakker}& $0.785$& $0.805$ \\
           \textbf{Uncertainty (Ours)} & $0.786$& $0.810$\\
           \midrule
           \textbf{0-step MSE Oracle} & $0.791$ & $0.819$\\
           \textbf{1-step SSIM Oracle} & $0.784$ & $0.816$\\
           \bottomrule
           \end{tabular}
           \captionof{table}{Average SSIM test set AUC (one AUC per image) on Knee 128.}\label{tab:comp_knee_ssim} 
    \end{center}
    \end{minipage}
    \end{figure}

==> figures/gan/tables/mnist_adaptive_grid.tex <==
\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $28.02$ & $27.89$ & $30.73$ & $--$\\
    & NC& $28.92$ & $34.98$ & $28.44$ & $--$\\
    & AO& $24.03$ & $19.82$ & $34.19$ & $--$\\
    \midrule
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $24.4$& $23.95$ & $22.83$& -\\
    & NC& $25.09$ & $25,35$ & $23.81$& $--$\\  
    & AO& $24,34$ & $24,21$ & $23.44$& -\\  
    & Zhang& $--$ & $--$ & $--$& $--$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{ResUNet table. Average PSNR test set AUC (one AUC per image) with on MNIST.}\label{tab:comp_mnist_psnr2} 
\end{center}
%Here mask embedding seems to do a diff but we report without it.

\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{0.96\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $0.90$ & $0.89$ & $0.92$ & -\\
    & NC& $0.91$ & $0.91$ & $0.90$ & -\\
    & AO& $0.90$ & $0.84$ & $0.94$ & -\\
    \midrule
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $0.55$& $0.54$ & $0.48$& -\\
    & NC& $0.59$ & $0.59$ & $0.53$& $--$\\  
    & AO& $0.56$ & $0.55$ & $0.5$& -\\  
    & Zhang& $--$ & $--$ & $--$& $--$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{ResUnet table. Average SSIM set AUC (one AUC per image) on MNIST.}\label{tab:comp_mnist_ssim2} 
\end{center}
\end{minipage}
\end{figure}

\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $28.33$ & $23.33$ & $24.45$ & -\\
    & NC& $26.92$ & $35.44$ & $27.78$ & -\\
    & AO& $23.82$ & $23.19$ & $27.98$ & -\\
    \midrule
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $24.34$& $24.90$ & $24.29$&  $20.45$\\
    & NC& $26.87$ & $28.93$ & $27.63$& $22.15$\\  
    & AO& $24.27$ & $25.08$ & $24.88$& $20.16$\\  
    & Zhang& $-$ & $-$ & $-$& $21.94$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{cResNet table. Average PSNR test set AUC (one AUC per image) with on MNIST.}\label{tab:comp_mnist_psnr2} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{0.96\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $0.91$ & $0.89$ & $0.90$ & -\\
    & NC& $0.91$ & $0.96$ & $0.93$ & -\\
    & AO& $0.87$ & $0.87$ & $0.92$ & -\\
    \midrule
    
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $0.6$& $0.57$ & $0.56$&$0.44$\\
    & NC& $0.79$ & $0.78$ & $0.77$& $0.52$\\  
    & AO& $0.61$ & $0.57$ & $0.57$& $0.43$\\  
    & Zhang& $-$ & $-$ & $-$& $0.52$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{cResNet table. Average SSIM set AUC (one AUC per image) on MNIST.}\label{tab:comp_mnist_ssim2} 
\end{center}
\end{minipage}
\end{figure}


==> figures/gan/tables/mnist_baseline.tex <==
\begin{center}
\begin{minipage}[t]{0.7\textwidth}

\input{files/gan/tables/mnist_new_image}
\end{minipage}\hfill
\end{center}
%\begin{minipage}[t]{0.48\textwidth}
%\input{tables/mnist_new_fourier}
%\end{minipage}

==> figures/gan/tables/mnist_comparison.tex <==
\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
    \resizebox{0.96\textwidth}{!}{\begin{tabular}{lccccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{7}{c}{\textbf{Model}}\\
    \cmidrule{2-8} & FAR & FWR & FNR & FAC & FWC & FNC & Zhang\\
    \midrule
    VDS & $21.75$  & $21.44$& $22.84$& $21.01$&$20.99$& $23.22$ &$23.94$\\
    LBC & $\mathbf{26.38}$ & $\mathbf{26.62}$& $\mathbf{27.77}$&$-$&$-$&$-$ & TODO\\
    Zhang Gaussian  &$-$ &$-$&&&&&$21.05$\\
    Zhang Evaluator  & -- & $-$&$-$&$20.45$&$22.15$&$20.16$ &$21.94$ \\
    Uncertainty (Ours) & $23.44$& $24.4$ &$25.35$&$24.88$&$24.34$&$28.93$& $27.72$ (FNR)\\
    \midrule
    MSE Oracle &$26.79$ &$-$ & $26.98$& $-$ &$-$& $-$&$-$\\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average PSNR test set AUC (one AUC per image) on MNIST (Fourier).}\label{tab:comp_mnist_psnr} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
     \resizebox{0.96\textwidth}{!}{\begin{tabular}{lccccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{7}{c}{\textbf{Model}}\\
    \cmidrule{2-8} & FAR & FWR & FNR & FAC & FWC & FNC & Zhang\\
    \midrule
    VDS & $0.52$  & $0.5$& $0.57$&$0.49$&$0.49$& $0.62$&$0.66$\\
    LBC & $0.58$ & $0.60$&$0.63$&$-$&$-$&$-$&TODO\\
    Zhang Gaussian  & $-$ & -- &&&&&$0.51$\\
    Zhang Evaluator & -- & $-$&$-$&$0.44$&$0.53$&$0.43$&$0.52$\\
    Uncertainty (Ours) & $0.5$ & $0.55$& $0.59$& $0.57$& $0.6$& $0.78$&$0.76$\\
    \midrule
    MSE Oracle & $0.63$& -- & $0.63$&&&&\\
    \end{tabular}}
    \captionof{table}{Average SSIM set AUC (one AUC per image) on MNIST (Fourier).}\label{tab:comp_mnist_ssim} 
\end{center}
\end{minipage}
\end{figure}

\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
    \resizebox{0.96\textwidth}{!}{\begin{tabular}{lcccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{6}{c}{\textbf{Model}}\\
    \cmidrule{2-7} & IAR & IWR & INR & IAC & IWC & INC\\
    \midrule
    VDS & $17.66$  & $17.27$& $17.65$&$17.14$&$16.4$& $17.28$\\
    LBC & $21.38$ & $21.42$&$22.95$&$-$&$-$&$-$\\
    Uncertainty (Ours) & $28.45$& $27.97$&$36.03$&$32.51$&$27.79$&$33.97$\\
    \midrule
    MSE Oracle &$44.57$ & $46.2$&$53.01$&&&\\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average PSNR test set AUC (one AUC per image) on MNIST (Image).}\label{tab:comp_mnist_psnr} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
     \resizebox{0.96\textwidth}{!}{\begin{tabular}{lcccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{6}{c}{\textbf{Model}}\\
    \cmidrule{2-7} & IAR & IWR & INR & IAC & IWC & INC \\
    \midrule
    VDS & $0.75$  &$0.76$&$0.78$&$0.74$&$0.75$&$0.79$ \\
    LBC & $0.91$ & $0.91$&$0.93$&$-$&$-$&$-$\\
    Uncertainty (Ours) & $0.93$ & $0.93$&$0.91$&$0.91$&$0.90$&$0.94$\\
    \midrule
    MSE Oracle & $0.98$& $0.87$&$0.98$&&&\\
    \end{tabular}}
    \captionof{table}{Average SSIM set AUC (one AUC per image) on MNIST (Image).}\label{tab:comp_mnist_ssim} 
\end{center}
\end{minipage}
\end{figure}

==> figures/gan/tables/mnist_new_fourier.tex <==
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lll|ccc}
    \toprule
    Algorithm & Model & Architecture & PSNR [dB]$~(\uparrow)$  &SSIM $(\uparrow)$& Accuracy  $ [\%]~(\uparrow)$\\
    \midrule
    \multirow{2}{*}{VDS}
     & NC &ResUNet& $21.61$  & $0.55$ & $0.84$ \\
     & WGAN &c-ResNet& $21.59$  & $0.57$ & $0.77$ \\    
    \midrule
    
    \multirow{4}{*}{LBC \cite{sanchez2019scalable}} 
     & NC & ResUNet & $25.61\pm 2.42$  & $0.60\pm 0.07$ & $0.97\pm 0.11$ \\
     & NC & c-ResNet& $25.79\pm 2.30$  & $0.63 \pm 0.07$ & $0.98 \pm 0.12$ \\
     & WGAN& ResUNet & $25.33 \pm 2.2$2   & $0.58\pm 0.06$ & $0.97\pm 0.12$ \\
     & WGAN& c-ResNet& $\mathbf{28.10\pm 2.08}$  & $\mathbf{0.78\pm 0.05}$ & $0.98 \pm 0.12$\\  
     
    \midrule
     \multicolumn{2}{l}{Zhang et al.\cite{zhang2019reducing}} &c-ResNet& $23.99 \pm 2.40$ & $0.74 \pm 0.07$& $0.96 \pm 0.14$\\
    \midrule
    \multirow{4}{*}{\begin{minipage}{1cm}GAS (Ours)\end{minipage}}  
     & NC&ResUNet & $25.02\pm 2.06$  & $0.60\pm 0.07$ & $0.98 \pm 0.12$ \\
     & NC& c-ResNet& $24.70\pm 2.50$  & $0.62 \pm 0.07$ & $0.98 \pm 0.12$ \\   
     & WGAN& ResUNet &  $24.19 \pm 1.95$  & $0.53 \pm 0.06$ & $0.97 \pm 0.12$ \\
     & WGAN& c-ResNet & $\mathbf{27.74 \pm 1.94}$  & $\mathbf{0.74\pm 0.06}$ & $0.98 \pm 0.12$ \\ 

    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC with standard deviation (one AUC per image) on MNIST, in Fourier domain.}\label{tab:comp_mnist_f}    


\begin{comment}
\resizebox{\textwidth}{!}{\begin{tabular}{ll|ccc}
    \toprule
    \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Model}  & PSNR  &SSIM & Accuracy  \\
    & & [dB]$~(\uparrow)$ &  $(\uparrow)$ &  $ [\%]~(\uparrow)$ \\
    \midrule
    \multirow{5}{*}{Baseline} 
     & FWR & $19.99$  & $0.47$  & $0.79$ \\
     & FNR & $20.96$  & $0.53$ & $0.81$ \\
     & FWC & $20.86$  & $0.55$ & $0.75$ \\    
     & FNC & $20.10$  & $0.50$  & $0.77$  \\  
    \midrule
    
    \multirow{5}{*}{LBC} 
     & FWR & $23.70 \pm 0.24$   & $0.53\pm 0.01$ & - \\
     & FNR & $24.17\pm 0.24$  & $0.57\pm 0.01$ & - \\
     & FWC & $\mathbf{26.35\pm 0.26}$  & $\mathbf{0.74\pm 0.01}$ & $0.92 \pm 0.004$\\  
     & FNC & $25.64\pm 0.61$  & $0.59 \pm 0.24$ & $0.92 \pm 0.004$ \\
    \midrule
    \multirow{5}{*}{GUD-ACS}  
     & FWR &  $23.59\pm 0.24$  & $0.52 \pm 0.01$ & $0.86 \pm 0.004$ \\
     & FNR & $24.41 \pm 0.25$  & $0.58\pm 0.01$ & $0.951 \pm 0.004$ \\
     & FWC & $\mathbf{27.01 \pm 0.27}$  & $\mathbf{0.74\pm 0.01}$ & $\mathbf{0.960 \pm 0.004}$ \\ 
     & FNC & $24.19 \pm 0.24$  & $0.61 \pm 0.01$ & $\mathbf{0.962 \pm 0.004}$ \\   
     \midrule
     \multicolumn{2}{l|}{Zhang baseline} & $21.83$& $0.61$ & $0.81$\\
     \multicolumn{2}{l|}{Zhang adaptive} & $23.44 \pm 0.24$ & $0.72 \pm 0.01$& $0.928 \pm 0.004$\\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC with standard deviation (one AUC per image) on MNIST, in Fourier domain.}\label{tab:comp_mnist_f}    
    \end{comment}


==> figures/gan/tables/mnist_new_image.tex <==
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lll|ccc}
    \toprule
    Algorithm & Model & Architecture & PSNR [dB]$~(\uparrow)$  &SSIM $(\uparrow)$& Accuracy  $ [\%]~(\uparrow)$\\
    \midrule
    \multirow{2}{*}{VDS} 
    & NC & ResUNet& $17.10$  & $0.76$ & $0.67$ \\
    & WGAN & c-ResNet & $16.41$  & $0.76$ & $0.67$ \\    
    \midrule
    \multirow{2}{*}{VDS} 
    & Recon. & ResUNet& $18.87\pm 2.31$  & $0.77\pm 0.05$ & $0.70\pm 0.21$ \\
    & Recon. & c-ResNet & $18.85\pm 2.18$  & $0.70\pm 0.05$ & $0.75\pm 0.20$ \\        
    \midrule
    \multirow{4}{*}{LBC \cite{sanchez2019scalable}}
     & NC &  ResUNet&$21.39 \pm 2.34$  & $0.90\pm 0.04$ & $0.92\pm 0.14$ \\
     & NC &  c-ResNet&$20.33\pm 2.20$  & $0.88 \pm 0.04$ & $0.93 \pm 0.15$ \\
     & WGAN & ResUNet& $20.29 \pm 2.09$  & $0.89 \pm 0.04$ & $0.90\pm 0.14$ \\
     & WGAN & c-ResNet& $20.48 \pm 2.14$  & $0.89\pm 0.04$ & $0.92\pm 0.14$\\
     
    \midrule
    \multirow{4}{*}{\begin{minipage}{1cm}GAS (Ours)\end{minipage}}
     & NC & ResUNet& $\mathbf{40.15 \pm 15.78}$  & $\mathbf{0.94\pm 0.04}$ & $0.91 \pm 0.15$ \\
     & NC & c-ResNet& $31.47 \pm 6.69$  & $0.93\pm 0.03$ & $\mathbf{0.93 \pm 0.14}$ \\       
     & WGAN & ResUNet& $31.73\pm 9.10$  & $0.92 \pm 0.06$ & $0.88 \pm 0.17$ \\
     & WGAN & c-ResNet& $\mathbf{35.81 \pm 10.34}$  & $\mathbf{0.96\pm 0.03}$ & $\mathbf{0.95\pm 0.13}$ \\    
     
     
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC (one AUC per image) with standard deviation on MNIST, in image domain.}\label{tab:comp_mnist_i}    

==> figures/pdm/comparison_algos/rates_radial_imspace.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=0.3,
xlabel style={font=\color{white!15!black}},
xlabel={Sampling rate},
ymin=26,
ymax=38,
ylabel style={font=\color{white!15!black}},
ylabel={PSNR},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.474,0.173)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark=x, mark options={solid, blue}]
  table[row sep=crcr]{%
0.025	27.382567668604\\
0.05	30.2617863537563\\
0.075	32.0700283097623\\
0.1	33.346928360636\\
0.125	34.3544222192726\\
0.15	35.0549438296553\\
0.175	35.7016662192604\\
0.2	35.8964406816977\\
0.225	36.0451978424498\\
0.25	36.3838608334005\\
0.275	36.6977770545573\\
0.3	37.3266248023346\\
};
\addlegendentry{$\text{Optimised x}_\text{i}$}

\addplot [color=red, mark=+, mark options={solid, red}]
  table[row sep=crcr]{%
0.025	27.0791791416404\\
0.05	29.2887721601854\\
0.075	30.8980186852358\\
0.1	32.0148147560125\\
0.125	33.062056834799\\
0.15	33.9366363372646\\
0.175	34.794594655969\\
0.2	35.7059256915435\\
0.225	36.3356450532064\\
0.25	36.5896122933467\\
0.275	36.6962853814378\\
0.3	36.9733584089672\\
};
\addlegendentry{$\text{Optimised Radial x}_{\text{radial,i}}$}

\addplot [color=black, dashed]
 plot [error bars/.cd, y dir = both, y explicit]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
0.025	30.873477401471	1.80895450013556	1.80895450013556\\
0.05	29.9991011019287	1.94790488558727	1.94790488558727\\
0.075	30.5218927834349	1.01474564565809	1.01474564565809\\
0.1	31.7225350294808	1.16057652108347	1.16057652108347\\
0.125	32.5523836015642	0.521037201246838	0.521037201246838\\
0.15	33.5938203447282	0.560240371853696	0.560240371853696\\
0.175	34.3564491014716	0.37972994977895	0.37972994977895\\
0.2	34.9813512657689	0.408439760388607	0.408439760388607\\
0.225	35.7064146161306	0.322107006009031	0.322107006009031\\
0.25	36.3441548505966	0.381182340612926	0.381182340612926\\
0.275	36.8324289072854	0.464567960243554	0.464567960243554\\
0.3	37.3696014559186	0.352796226644492	0.352796226644492\\
};
\addlegendentry{Random}

\end{axis}
\end{tikzpicture}%

==> figures/pdm/comparison_algos/rates_radial_kspace.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.602in,
height=3.566in,
at={(0.772in,0.481in)},
scale only axis,
xmin=0,
xmax=0.3,
xlabel style={font=\color{white!15!black}},
xlabel={Sampling rate},
ymin=26,
ymax=38,
ylabel style={font=\color{white!15!black}},
ylabel={PSNR},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.52,0.161)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark=x, mark options={solid, blue}]
  table[row sep=crcr]{%
0.025	27.3332997697084\\
0.05	30.1998127095317\\
0.075	31.9802823358828\\
0.1	33.2266730346306\\
0.125	34.1988144184603\\
0.15	34.8612831898287\\
0.175	35.4714111080465\\
0.2	35.6269092040207\\
0.225	35.7560469738236\\
0.25	36.0612698671979\\
0.275	36.3347039866566\\
};
\addlegendentry{$\text{Optimised x}_\text{i}$}

\addplot [color=red, mark=+, mark options={solid, red}]
  table[row sep=crcr]{%
0.025	27.0217154847296\\
0.05	29.2228536115997\\
0.075	30.7952657729741\\
0.1	31.8803307930429\\
0.125	32.8873298146683\\
0.15	33.744794368452\\
0.175	34.5644880771616\\
0.2	35.4459843290354\\
0.225	36.0543596249987\\
0.25	36.2817574432956\\
0.275	36.3455931291089\\
0.3	36.5827961686373\\
};
\addlegendentry{$\text{Optimised Radial x}_{\text{radial,i}}$}

\addplot [color=black, dashed]
 plot [error bars/.cd, y dir = both, y explicit]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
0.025	29.649762675288	1.99001689731684	1.99001689731684\\
0.05	29.7930011709283	1.6872644267804	1.6872644267804\\
0.075	30.4388558892866	1.48947541757156	1.48947541757156\\
0.1	31.4489488264075	1.25151792477212	1.25151792477212\\
0.125	32.4130835349112	0.81041265507179	0.81041265507179\\
0.15	33.2961244384302	0.420807468828699	0.420807468828699\\
0.175	34.1440870959689	0.464636734739712	0.464636734739712\\
0.2	34.7751221909502	0.336686304169435	0.336686304169435\\
0.225	35.4832875869528	0.380400152707237	0.380400152707237\\
0.25	36.0612413459803	0.367336969985818	0.367336969985818\\
0.275	36.607285881972	0.387514114260523	0.387514114260523\\
0.3	36.9459442790928	0.306796209823419	0.306796209823419\\
};
\addlegendentry{Random}

\end{axis}
\end{tikzpicture}%

==> figures/rethinking_pmri/sense_aloha_pmri_masks.tex <==
\begin{tabular}{cccc}
    & \hspace{-5mm} \textbf{{Mask}} & \hspace{-4mm} \textbf{{SENSE }} & \hspace{-4mm} \textbf{{ALOHA }}    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hspace{-2mm} \rotatebox{90}{\hspace{2mm} \textbf{{Coher. based}}} &                         
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/coherence_20.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_coherence.pdf}  & 
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_coherence.pdf}  \\ [-1mm]
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hspace{-1mm} \rotatebox{90}{\hspace{7mm} \textbf{{TV LB}}} &
    %\hspace{-5mm}\includegraphics[width=.15\textwidth]{FIGURES_NEW/baran/mask_SSI20M.pdf} &
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/TV_20.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_TV.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_TV.pdf}   \\ [-1mm]
    
    % & 6.25\% sampling & 12.5\% sampling & 25\% sampling \\ 
    
    \hspace{-1mm}\rotatebox{90}{\hspace{7mm} \textbf{{BP LB}}} &                         
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/BP_shearlet_20.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_BP_shearlet.pdf}  & 
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_BP_shearlet.pdf}  \\ [-1mm]
    % & 6.25\% sampling & 12.5\% sampling & 25\% sampling \\ 
    
    \hspace{-1mm}\rotatebox{90}{\hspace{1mm} \textbf{{SENSE LB-VD}}} &                         
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/SENSE_LB1_20.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_SENSE_LB1.pdf}  & 
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_SENSE_LB1.pdf}  \\ [-1mm]
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \hspace{-1mm}\rotatebox{90}{\hspace{0mm} \textbf{{ALOHA LB-VD}}} &                         
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/ALOHA_LB1_20.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_ALOHA_LB1.pdf}  & 
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_ALOHA_LB1.pdf}  \\ [-1mm]
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \hspace{-1mm}\rotatebox{90}{\hspace{4mm} \textbf{{SENSE LB}}} &                         
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/SENSE_LB2_20.pdf} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_SENSE_LB2.pdf}  & 
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_SENSE_LB2.pdf}  \\ [-1mm]
    
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \hspace{-1mm}\rotatebox{90}{\hspace{3mm} \textbf{{ALOHA LB}}} &                         
    \hspace{-2mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/ALOHA_LB2_20.PDF} &
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_BART-SENSE_ALOHA_LB2.pdf}  & 
    \hspace{-4mm}\includegraphics[width=.15\textwidth]{figures/rethinking_pmri/MULTI_index_95_rate_20_algo_and_mask_LRH_ALOHA_LB2.pdf}  \\ [-1mm]
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}

==> figures/rethinking_pmri/sense_pmri_masks_recon.tex <==
%\tiny
\begin{tabular}{ccc}
    & \textbf{Masks} & \textbf{Recon} \\

    \rotatebox{90}{\parbox{.45\linewidth}{\textbf{Fully\\ sampled}}}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/kspace_19.pdf} 
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/original_19.pdf} \\
    \rotatebox{90}{\textbf{\tiny CAIPIRINHA}}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/CAIRIPINHA_mask.pdf}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/CAIRIPINHA_recon.pdf} \\
    \rotatebox{90}{\parbox{.45\linewidth}{\textbf{Poisson\\ Disk}}}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/poisson_disk_uniform_mask.pdf}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/poisson_disk_uniform_recon.pdf} \\
    \rotatebox{90}{\parbox{.45\linewidth}{\textbf{Adaptive\\ random}}}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/AR_mask.pdf}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/AR_recon} \\
    \rotatebox{90}{\textbf{VD-PD}}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/poisson_disk_mask.pdf}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/poisson_disk_recon.pdf} \\
    \rotatebox{90}{\textbf{lLBCS}}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/LBL_mask.pdf}
    & \includegraphics[width=.45\linewidth]{figures/rethinking_pmri/LBL_recon} \\
\end{tabular}

==> figures/simple_baselines/tables/bakker_knee_table.tex <==
\begin{figure}[h]
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
         \toprule
        \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
        \midrule
        \textbf{Random} & $24.22$ & $20.68$ \\
        \textbf{LtH} & $24.25$ & $23.63$\\
        \textbf{LBCS} & $24.57$& $23.82$\\
        \textbf{NA Oracle}& $24.56$& $23.82$\\           
        \textbf{Bakker} & $24.37$& $22.50$ \\
        \bottomrule
        \end{tabular}
        \captionof{table}{Average PSNR test set AUC (one AUC per image) on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_psnr}     \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
            \toprule
           \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
           \midrule
            \textbf{Random}& $0.6251$& $0.5557$ \\
            \textbf{LtH}& $0.6073$& $0.5687$\\
            \textbf{LBCS}& $0.6355$& $0.5894$\\
            \textbf{NA Oracle}& $0.6355$& $0.5886$\\           
            \textbf{Bakker}& $0.6387$& $0.6153$ \\
           \bottomrule
           \end{tabular}
           \captionof{table}{Average SSIM test set AUC (one AUC per image) on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_ssim} 
    \end{center}
    \end{minipage}
    \end{figure}
    
    
    
    \begin{figure}[h]
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
         \toprule
        \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
        \midrule
        \textbf{Random} & $24.84$ & $21.66$ \\
        \textbf{LtH} & $24.81$ & $24.81$\\
        \textbf{LBCS} & $25.40$& $25.40$\\
        \textbf{NA Oracle}& $25.39$& $25.40$\\           
        \textbf{Bakker} & $25.18$& $24.60$ \\
        \bottomrule
        \end{tabular}
        \captionof{table}{Average PSNR at $25\%$ on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_psnr_25}     \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
            \toprule
           \multirow{1}{*}{\textbf{Policy}}& Base horizon& Long horizon\\
           \midrule
            \textbf{Random}& $0.6896$& $0.6589$ \\
            \textbf{LtH}& $0.6586$& $0.6586$\\
            \textbf{LBCS}& $0.7086$& $0.7095$\\
            \textbf{NA Oracle}& $0.7099$& $0.7097$\\           
            \textbf{Bakker}& $0.7165$& $0.7400$ \\
           \bottomrule
           \end{tabular}
           \captionof{table}{Average SSIM at $25\%$ on Bakker 128x128 knee setting.}\label{tab:bakker_comp_knee_ssim_25} 
    \end{center}
    \end{minipage}
    \end{figure}

==> figures/simple_baselines/tables/bakker_tables/bakker_mismatched_ablation_ssim_auc_sh.tex <==
\begin{tabular}{lccccc}
\toprule
\textbf{Policy} & \textbf{Bakker's setting} & \textbf{Individual data range} & \textbf{Data standardization} & \textbf{Mismatched setting} & \textbf{Our preprocessing} \\
\midrule
\textbf{Random (SH)} & 0.6251 & 0.5964 & 0.5798 & 0.5595 & 0.5608 \\
\textbf{LtH (SH)} & 0.6073 & 0.5762 & 0.565 & 0.5617 & 0.5719 \\
\textbf{LBCS (SH)} & 0.6375 & 0.6099 & 0.5928 & 0.5707 & 0.5732 \\
\textbf{RL (SH) - eval} & 0.6388 & 0.6112 & 0.5941 & 0.5698 & 0.5738 \\
\textbf{NA Oracle (SH)} & 0.6383 & 0.6107 & 0.5937 & 0.5717 & 0.5738\\
\bottomrule
\end{tabular}

==> figures/simple_baselines/tables/bakker_tables/bakker_mismatched_at_25_ssim.tex <==
\begin{tabular}{lccc}
 \toprule
\textbf{Policy}& Bakker prepro  & Mismatched prepro & Our prepro\\
\midrule
\textbf{Random} & $0.6465\pm 0.0003$ &  $0.6107\pm 0.0003$ & $0.607$\\
\textbf{LtH} & $0.6143$ & $0.6123$ & $0.6267$\\
\textbf{LBCS} & $0.6734 \pm 0.0002$ & $0.6269 \pm 0.0006$ & $0.6288$\\
\textbf{RL} & $\mathbf{0.6751\pm 0.0001}$& $\mathbf{0.6286 \pm 0.0001}$ &$\mathbf{0.6298}$\\
\midrule
\textbf{NA Oracle} & $0.6745$ & $0.633$& $0.6301$\\

\bottomrule
\end{tabular}
      

==> figures/simple_baselines/tables/bakker_tables/bakker_mismatched_auc_ssim.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Policy}& Bakker prepro  & Mismatched prepro & Our prepro\\
\midrule
\textbf{Random} & $0.5798\pm 0.0002$ &  $0.5595\pm 0.0002$ & $0.5608$\\
\textbf{LtH} & $0.5610$ & $0.5584$ & $0.5719$\\
\textbf{LBCS} & $0.5931 \pm 0.0002$ & $0.5684 \pm 0.0005$ & $0.5732$\\
\textbf{RL} & $\mathbf{0.5942\pm 0.0001}$& $\mathbf{0.5697 \pm 0.0001}$ &$\mathbf{0.5738}$\\
\midrule
\textbf{NA Oracle} & $0.5937$ & $0.5717$& $0.5738$\\
\bottomrule
\end{tabular}
      

==> figures/simple_baselines/tables/bakker_tables/bakker_mismatched_undersampled_auc.tex <==
\begin{tabular}{lcc}
 \toprule
 
\textbf{Policy}& Bakker prepro  & Our prepro \\
\midrule
\textbf{Random} & $0.5633\pm 0.0002$ &  $0.5510\pm 0.0002$\\
\textbf{LtH} & $0.5714$ & $0.5665$\\
\textbf{LBCS} & $0.5706 \pm 0.0003$ & $\mathbf{0.5619 \pm 0.0008}$\\
\textbf{RL} & $\mathbf{0.5736\pm 0.0001}$& $0.5967 \pm 0.0001$ &$\mathbf{0.5599}$\\
\midrule
\textbf{NA Oracle} & $0.5716$ & $0.5632$& $0.5738$\\

\bottomrule
\end{tabular}
      
%The results on undersampled are not as compelling as I would have wished. They aren't that informative and maybe we could get more out of illustrating this difference in the actual Bakker experiment?

==> figures/simple_baselines/tables/brain_sampling.tex <==
\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
    \begin{tabular}{lcc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{2}{c}{\textbf{Model}}\\
    \cmidrule{2-3} & AO & Zhang\\
    \midrule
    VDS & $31.7$1& $28.78$ \\
    LBCS & $\mathbf{34.03}$& $\mathbf{32.03}$\\
    Zhang Gaussian  & - & $25.37$\\
    Zhang Evaluator & $32.19$& $29.95$\\
    Bakker & $31.45$& $28.23$ \\
    Uncertainty (Ours) & $33.77$& $31.18$\\
    \midrule
    MSE Oracle &$34.21$ & $30.69$\\
    \bottomrule
    \end{tabular}
    \captionof{table}{Average PSNR test set AUC (one AUC per image) on Brain 256.}\label{tab:comp_brain_psnr} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
     \begin{tabular}{lcc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{2}{c}{\textbf{Model}}\\
    \cmidrule{2-3} &AO & Zhang\\
    \midrule
    VDS & $0.82$ &$0.82$ \\
    LBCS &  $\mathbf{0.88}$& $0.84$\\
    Zhang Gaussian & - & $0.72$\\
    Zhang Evaluator & $0.83$& $0.85$\\
    Bakker &$0.80$ & $0.80$\\
    Uncertainty (Ours) & $\mathbf{0.88}$ & $\mathbf{0.87}$\\
    \midrule
    MSE Oracle & $0.89$& $0.87$\\
    \end{tabular}
    \captionof{table}{Average SSIM set AUC (one AUC per image) on Brain 256.}\label{tab:comp_brain_ssim} 
\end{center}
\end{minipage}
\end{figure}

==> figures/simple_baselines/tables/cifar_baseline.tex <==
\begin{center}
\begin{minipage}[t]{0.7\textwidth}

\input{tables/cifar_image}
\end{minipage}\hfill
\end{center}

==> figures/simple_baselines/tables/cifar_image.tex <==
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lll|ccc}
    \toprule
    Algorithm & Model & Architecture & PSNR [dB]$~(\uparrow)$  &SSIM $(\uparrow)$& Accuracy  $ [\%]~(\uparrow)$\\
    \midrule
    \multirow{2}{*}{VDS} 
    & NC & ResUNet& $9.32\pm 0.70$  & $0.11\pm0.03$ & $0.10\pm 0.17$ \\
    & WGAN & ResUNet & $8.72\pm 0.62$  & $0.09\pm 0.03$ & $0.10\pm 0.17$ \\    
    \midrule
    \multirow{2}{*}{VDS}  & Recon. & ResUNet& $6.73\pm 0.51$  & $0.09\pm 0.02$ & $0.11\pm0.17$  \\
     & Recon. & c-ResNet& $ 11.79 \pm 0.72$  & $0.13 \pm 0.03$& $0.10\pm0.16$ \\
    \midrule
    \multirow{2}{*}{\begin{minipage}{1cm}GAS (Ours)\end{minipage}}
     & NC & ResUNet& $14.36 \pm 1.89$  & $0.55\pm 0.08$ & $\mathbf{0.27 \pm 0.22}$ \\
     & WGAN & ResUNet& $\mathbf{15.26\pm 2.34}$  & $\mathbf{0.57 \pm 0.09}$ & $0.21 \pm 0.18$ \\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC (one AUC per image) with standard deviation on CIFAR10, in image domain. This was computed on a subset of the test set.}\label{tab:comp_cifar_i}    

==> figures/simple_baselines/tables/knee_extended_table.tex <==
\begin{figure}[h]
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
         \toprule
        \multirow{1}{*}{\textbf{Policy}}& \multicolumn{2}{c}{\textbf{Model}}\\
        \cmidrule{2-3} & AO & Zhang\\
        \midrule
        \textbf{LtH} & $32.38$ & $31.97$\\
        \textbf{VDS} & $32.17$ & $31.29$ \\
        \textbf{LtH-VDS} & $32.94$ & $31.94$ \\
        \textbf{LBCS} & $33.40$& $32.13$\\
        \textbf{Zhang Evaluator} & $31.14$& $31.58$\\
        \textbf{Bakker} & $32.39$& $31.49$ \\
        \textbf{Uncertainty (Ours)} & $32.36$& $31.75$\\
        \midrule
        \textbf{0-step MSE Oracle} & $32.58$ & $32.18$\\
        \textbf{1-step SSIM Oracle} & $32.23$ & $32.24$\\
        \bottomrule
        \end{tabular}
        \captionof{table}{Average PSNR test set AUC (one AUC per image) on Knee 128.}\label{tab:comp_knee_psnr} 
    \end{center}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
    \begin{center}
        \begin{tabular}{lcc}
            \toprule
           \multirow{1}{*}{\textbf{Policy}}& \multicolumn{2}{c}{\textbf{Model}}\\
           \cmidrule{2-3} & AO & Zhang\\
           \midrule
           \textbf{LtH}& $0.785$& $0.813$\\
           \textbf{VDS}& $0.792$& $0.795$ \\
           \textbf{LtH-VDS}& $0.805$ & $0.808$ \\
           \textbf{LBCS}& $0.815$& $0.813$\\
           \textbf{Zhang Evaluator}& $0.759$& $0.802$\\
           \textbf{Bakker}& $0.785$& $0.805$ \\
           \textbf{Uncertainty (Ours)} & $0.786$& $0.810$\\
           \midrule
           \textbf{0-step MSE Oracle} & $0.791$ & $0.819$\\
           \textbf{1-step SSIM Oracle} & $0.784$ & $0.816$\\
           \bottomrule
           \end{tabular}
           \captionof{table}{Average SSIM test set AUC (one AUC per image) on Knee 128.}\label{tab:comp_knee_ssim} 
    \end{center}
    \end{minipage}
    \end{figure}

==> figures/simple_baselines/tables/mnist_adaptive_grid.tex <==
\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $28.02$ & $27.89$ & $30.73$ & $--$\\
    & NC& $28.92$ & $34.98$ & $28.44$ & $--$\\
    & AO& $24.03$ & $19.82$ & $34.19$ & $--$\\
    \midrule
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $24.4$& $23.95$ & $22.83$& -\\
    & NC& $25.09$ & $25,35$ & $23.81$& $--$\\  
    & AO& $24,34$ & $24,21$ & $23.44$& -\\  
    & Zhang& $--$ & $--$ & $--$& $--$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{ResUNet table. Average PSNR test set AUC (one AUC per image) with on MNIST.}\label{tab:comp_mnist_psnr2} 
\end{center}
%Here mask embedding seems to do a diff but we report without it.

\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{0.96\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $0.90$ & $0.89$ & $0.92$ & -\\
    & NC& $0.91$ & $0.91$ & $0.90$ & -\\
    & AO& $0.90$ & $0.84$ & $0.94$ & -\\
    \midrule
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $0.55$& $0.54$ & $0.48$& -\\
    & NC& $0.59$ & $0.59$ & $0.53$& $--$\\  
    & AO& $0.56$ & $0.55$ & $0.5$& -\\  
    & Zhang& $--$ & $--$ & $--$& $--$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{ResUnet table. Average SSIM set AUC (one AUC per image) on MNIST.}\label{tab:comp_mnist_ssim2} 
\end{center}
\end{minipage}
\end{figure}

\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $28.33$ & $23.33$ & $24.45$ & -\\
    & NC& $26.92$ & $35.44$ & $27.78$ & -\\
    & AO& $23.82$ & $23.19$ & $27.98$ & -\\
    \midrule
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $24.34$& $24.90$ & $24.29$&  $20.45$\\
    & NC& $26.87$ & $28.93$ & $27.63$& $22.15$\\  
    & AO& $24.27$ & $25.08$ & $24.88$& $20.16$\\  
    & Zhang& $-$ & $-$ & $-$& $21.94$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{cResNet table. Average PSNR test set AUC (one AUC per image) with on MNIST.}\label{tab:comp_mnist_psnr2} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{0.96\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Recon. model}}& \multicolumn{4}{c}{\textbf{Sampling Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{3}{*}{\textbf{Image}}& WGAN& $0.91$ & $0.89$ & $0.90$ & -\\
    & NC& $0.91$ & $0.96$ & $0.93$ & -\\
    & AO& $0.87$ & $0.87$ & $0.92$ & -\\
    \midrule
    
    \multirow{4}{*}{\textbf{Fourier}}& WGAN& $0.6$& $0.57$ & $0.56$&$0.44$\\
    & NC& $0.79$ & $0.78$ & $0.77$& $0.52$\\  
    & AO& $0.61$ & $0.57$ & $0.57$& $0.43$\\  
    & Zhang& $-$ & $-$ & $-$& $0.52$\\  
    \bottomrule
    \end{tabular}
    }\captionof{table}{cResNet table. Average SSIM set AUC (one AUC per image) on MNIST.}\label{tab:comp_mnist_ssim2} 
\end{center}
\end{minipage}
\end{figure}


==> figures/simple_baselines/tables/mnist_baseline.tex <==
\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Architecture}}& \multicolumn{4}{c}{\textbf{Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{2}{*}{\textbf{Image}}& ResUnet& $17.27$ & $17.65$ & $17,66$ & -\\
    & cResNet& $16,4$ & $17,28$ & $17,14$ & -\\
    \multirow{2}{*}{\textbf{Fourier}}& ResUnet& $21,44$& $22,84$ & $21,75$& -\\
    & cResNet& $20,99$ & $23,22$ & $21,01$& $23.94$\\    
    
    \bottomrule
    \end{tabular}
    }\captionof{table}{Average PSNR test set AUC (one AUC per image) with on MNIST.}\label{tab:baseline_mnist_psnr} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
\resizebox{0.96\textwidth}{!}{
    \begin{tabular}{llcccc}
     \toprule
    \multirow{2}{*}{\textbf{Domain}}&\multirow{2}{*}{\textbf{Architecture}}& \multicolumn{4}{c}{\textbf{Model}}\\
    \cmidrule{3-6} && WGAN & NC & AO & Zhang\\
    \midrule
    \multirow{2}{*}{\textbf{Image}}& ResUnet& $0.76$& $0.78$ & $0.76$ & -\\
    & cResNet& $0,75$ & $0,79$& $0,74$ & -\\
    \multirow{2}{*}{\textbf{Fourier}}& ResUnet& $0,5$& $0,57$ & $0,52$ &- \\
    & cResNet& $0,49$& $0.62$ & $0,49$ & $0.66$\\    
    \bottomrule
    \end{tabular}
    }\captionof{table}{Average SSIM set AUC (one AUC per image) on MNIST.}\label{tab:baseline_mnist_ssim} 
\end{center}
\end{minipage}
\end{figure}

==> figures/simple_baselines/tables/mnist_comparison.tex <==
\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
    \resizebox{0.96\textwidth}{!}{\begin{tabular}{lccccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{7}{c}{\textbf{Model}}\\
    \cmidrule{2-8} & FAR & FWR & FNR & FAC & FWC & FNC & Zhang\\
    \midrule
    VDS & $21.75$  & $21.44$& $22.84$& $21.01$&$20.99$& $23.22$ &$23.94$\\
    LBC & $\mathbf{26.38}$ & $\mathbf{26.62}$& $\mathbf{27.77}$&$-$&$-$&$-$ & TODO\\
    Zhang Gaussian  &$-$ &$-$&&&&&$21.05$\\
    Zhang Evaluator  & -- & $-$&$-$&$20.45$&$22.15$&$20.16$ &$21.94$ \\
    Uncertainty (Ours) & $23.44$& $24.4$ &$25.35$&$24.88$&$24.34$&$28.93$& $27.72$ (FNR)\\
    \midrule
    MSE Oracle &$26.79$ &$-$ & $26.98$& $-$ &$-$& $-$&$-$\\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average PSNR test set AUC (one AUC per image) on MNIST (Fourier).}\label{tab:comp_mnist_psnr} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
     \resizebox{0.96\textwidth}{!}{\begin{tabular}{lccccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{7}{c}{\textbf{Model}}\\
    \cmidrule{2-8} & FAR & FWR & FNR & FAC & FWC & FNC & Zhang\\
    \midrule
    VDS & $0.52$  & $0.5$& $0.57$&$0.49$&$0.49$& $0.62$&$0.66$\\
    LBC & $0.58$ & $0.60$&$0.63$&$-$&$-$&$-$&TODO\\
    Zhang Gaussian  & $-$ & -- &&&&&$0.51$\\
    Zhang Evaluator & -- & $-$&$-$&$0.44$&$0.53$&$0.43$&$0.52$\\
    Uncertainty (Ours) & $0.5$ & $0.55$& $0.59$& $0.57$& $0.6$& $0.78$&$0.76$\\
    \midrule
    MSE Oracle & $0.63$& -- & $0.63$&&&&\\
    \end{tabular}}
    \captionof{table}{Average SSIM set AUC (one AUC per image) on MNIST (Fourier).}\label{tab:comp_mnist_ssim} 
\end{center}
\end{minipage}
\end{figure}

\begin{figure}[h]
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
    \resizebox{0.96\textwidth}{!}{\begin{tabular}{lcccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{6}{c}{\textbf{Model}}\\
    \cmidrule{2-7} & IAR & IWR & INR & IAC & IWC & INC\\
    \midrule
    VDS & $17.66$  & $17.27$& $17.65$&$17.14$&$16.4$& $17.28$\\
    LBC & $21.38$ & $21.42$&$22.95$&$-$&$-$&$-$\\
    Uncertainty (Ours) & $28.45$& $27.97$&$36.03$&$32.51$&$27.79$&$33.97$\\
    \midrule
    MSE Oracle &$44.57$ & $46.2$&$53.01$&&&\\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average PSNR test set AUC (one AUC per image) on MNIST (Image).}\label{tab:comp_mnist_psnr} 
\end{center}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
\begin{center}
     \resizebox{0.96\textwidth}{!}{\begin{tabular}{lcccccc}
     \toprule
    \multirow{1}{*}{\textbf{Policy}}& \multicolumn{6}{c}{\textbf{Model}}\\
    \cmidrule{2-7} & IAR & IWR & INR & IAC & IWC & INC \\
    \midrule
    VDS & $0.75$  &$0.76$&$0.78$&$0.74$&$0.75$&$0.79$ \\
    LBC & $0.91$ & $0.91$&$0.93$&$-$&$-$&$-$\\
    Uncertainty (Ours) & $0.93$ & $0.93$&$0.91$&$0.91$&$0.90$&$0.94$\\
    \midrule
    MSE Oracle & $0.98$& $0.87$&$0.98$&&&\\
    \end{tabular}}
    \captionof{table}{Average SSIM set AUC (one AUC per image) on MNIST (Image).}\label{tab:comp_mnist_ssim} 
\end{center}
\end{minipage}
\end{figure}

==> figures/simple_baselines/tables/mnist_new_fourier.tex <==
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lll|ccc}
    \toprule
    Algorithm & Model & Architecture & PSNR [dB]$~(\uparrow)$  &SSIM $(\uparrow)$& Accuracy  $ [\%]~(\uparrow)$\\
    \midrule
    \multirow{2}{*}{VDS}
     & NC &ResUNet& $21.61$  & $0.55$ & $0.84$ \\
     & WGAN &c-ResNet& $21.59$  & $0.57$ & $0.77$ \\    
    \midrule
    
    \multirow{4}{*}{LBC \cite{sanchez2019scalable}} 
     & NC & ResUNet & $25.61\pm 2.42$  & $0.60\pm 0.07$ & $0.97\pm 0.11$ \\
     & NC & c-ResNet& $25.79\pm 2.30$  & $0.63 \pm 0.07$ & $0.98 \pm 0.12$ \\
     & WGAN& ResUNet & $25.33 \pm 2.2$2   & $0.58\pm 0.06$ & $0.97\pm 0.12$ \\
     & WGAN& c-ResNet& $\mathbf{28.10\pm 2.08}$  & $\mathbf{0.78\pm 0.05}$ & $0.98 \pm 0.12$\\  
     
    \midrule
     \multicolumn{2}{l}{Zhang et al.\cite{zhang2019reducing}} &c-ResNet& $23.99 \pm 2.40$ & $0.74 \pm 0.07$& $0.96 \pm 0.14$\\
    \midrule
    \multirow{4}{*}{\begin{minipage}{1cm}GAS (Ours)\end{minipage}}  
     & NC&ResUNet & $25.02\pm 2.06$  & $0.60\pm 0.07$ & $0.98 \pm 0.12$ \\
     & NC& c-ResNet& $24.70\pm 2.50$  & $0.62 \pm 0.07$ & $0.98 \pm 0.12$ \\   
     & WGAN& ResUNet &  $24.19 \pm 1.95$  & $0.53 \pm 0.06$ & $0.97 \pm 0.12$ \\
     & WGAN& c-ResNet & $\mathbf{27.74 \pm 1.94}$  & $\mathbf{0.74\pm 0.06}$ & $0.98 \pm 0.12$ \\ 

    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC with standard deviation (one AUC per image) on MNIST, in Fourier domain.}\label{tab:comp_mnist_f}    


\begin{comment}
\resizebox{\textwidth}{!}{\begin{tabular}{ll|ccc}
    \toprule
    \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Model}  & PSNR  &SSIM & Accuracy  \\
    & & [dB]$~(\uparrow)$ &  $(\uparrow)$ &  $ [\%]~(\uparrow)$ \\
    \midrule
    \multirow{5}{*}{Baseline} 
     & FWR & $19.99$  & $0.47$  & $0.79$ \\
     & FNR & $20.96$  & $0.53$ & $0.81$ \\
     & FWC & $20.86$  & $0.55$ & $0.75$ \\    
     & FNC & $20.10$  & $0.50$  & $0.77$  \\  
    \midrule
    
    \multirow{5}{*}{LBC} 
     & FWR & $23.70 \pm 0.24$   & $0.53\pm 0.01$ & - \\
     & FNR & $24.17\pm 0.24$  & $0.57\pm 0.01$ & - \\
     & FWC & $\mathbf{26.35\pm 0.26}$  & $\mathbf{0.74\pm 0.01}$ & $0.92 \pm 0.004$\\  
     & FNC & $25.64\pm 0.61$  & $0.59 \pm 0.24$ & $0.92 \pm 0.004$ \\
    \midrule
    \multirow{5}{*}{GUD-ACS}  
     & FWR &  $23.59\pm 0.24$  & $0.52 \pm 0.01$ & $0.86 \pm 0.004$ \\
     & FNR & $24.41 \pm 0.25$  & $0.58\pm 0.01$ & $0.951 \pm 0.004$ \\
     & FWC & $\mathbf{27.01 \pm 0.27}$  & $\mathbf{0.74\pm 0.01}$ & $\mathbf{0.960 \pm 0.004}$ \\ 
     & FNC & $24.19 \pm 0.24$  & $0.61 \pm 0.01$ & $\mathbf{0.962 \pm 0.004}$ \\   
     \midrule
     \multicolumn{2}{l|}{Zhang baseline} & $21.83$& $0.61$ & $0.81$\\
     \multicolumn{2}{l|}{Zhang adaptive} & $23.44 \pm 0.24$ & $0.72 \pm 0.01$& $0.928 \pm 0.004$\\
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC with standard deviation (one AUC per image) on MNIST, in Fourier domain.}\label{tab:comp_mnist_f}    
    \end{comment}


==> figures/simple_baselines/tables/mnist_new_image.tex <==
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lll|ccc}
    \toprule
    Algorithm & Model & Architecture & PSNR [dB]$~(\uparrow)$  &SSIM $(\uparrow)$& Accuracy  $ [\%]~(\uparrow)$\\
    \midrule
    \multirow{2}{*}{VDS} 
    & NC & ResUNet& $17.10$  & $0.76$ & $0.67$ \\
    & WGAN & c-ResNet & $16.41$  & $0.76$ & $0.67$ \\    
    \midrule
    \multirow{2}{*}{VDS} 
    & Recon. & ResUNet& $18.87\pm 2.31$  & $0.77\pm 0.05$ & $0.70\pm 0.21$ \\
    & Recon. & c-ResNet & $18.85\pm 2.18$  & $0.70\pm 0.05$ & $0.75\pm 0.20$ \\        
    \midrule
    \multirow{4}{*}{LBC \cite{sanchez2019scalable}}
     & NC &  ResUNet&$21.39 \pm 2.34$  & $0.90\pm 0.04$ & $0.92\pm 0.14$ \\
     & NC &  c-ResNet&$20.33\pm 2.20$  & $0.88 \pm 0.04$ & $0.93 \pm 0.15$ \\
     & WGAN & ResUNet& $20.29 \pm 2.09$  & $0.89 \pm 0.04$ & $0.90\pm 0.14$ \\
     & WGAN & c-ResNet& $20.48 \pm 2.14$  & $0.89\pm 0.04$ & $0.92\pm 0.14$\\
     
    \midrule
    \multirow{4}{*}{\begin{minipage}{1cm}GAS (Ours)\end{minipage}}
     & NC & ResUNet& $\mathbf{40.15 \pm 15.78}$  & $\mathbf{0.94\pm 0.04}$ & $0.91 \pm 0.15$ \\
     & NC & c-ResNet& $31.47 \pm 6.69$  & $0.93\pm 0.03$ & $\mathbf{0.93 \pm 0.14}$ \\       
     & WGAN & ResUNet& $31.73\pm 9.10$  & $0.92 \pm 0.06$ & $0.88 \pm 0.17$ \\
     & WGAN & c-ResNet& $\mathbf{35.81 \pm 10.34}$  & $\mathbf{0.96\pm 0.03}$ & $\mathbf{0.95\pm 0.13}$ \\    
     
     
    \bottomrule
    \end{tabular}}
    \captionof{table}{Average test set AUC (one AUC per image) with standard deviation on MNIST, in image domain.}\label{tab:comp_mnist_i}    

==> figures/simple_baselines/tables/pineda_tables/pineda_100.tex <==
\begin{tabular}{lcc}
 \toprule
\multirow{1}{*}{\textbf{Policy}}& SSIM& PSNR\\
\midrule
\textbf{Random} & $0.6723$ &  $28.962$ \\
%\textbf{Random low bias} & $0.6847$ & $29.974$ \\
\textbf{LtH} & $0.6686$ & $29.360$\\
\textbf{LBCS} & $\mathbf{0.6886}$ & $\mathbf{ 30.211}$\\
\textbf{Evaluator} & $0.6812$& $29.681$ \\
\textbf{DS-DDQN} & $0.6855$& $29.652$ \\
\textbf{SS-DDQN} & $0.6882$& $29.929$ \\
\midrule
\textbf{Oracle} & $0.7131$ & $30.683$\\

\bottomrule
\end{tabular}
